A Black-Box Approach to Post-Quantum Zero-Knowledge in Constant Rounds

In a recent seminal work, Bitansky and Shmueli (STOC '20) gave the first construction of a constant round zero-knowledge argument for NP secure against quantum attacks. However, their construction has several drawbacks compared to the classical counterparts. Specifically, their construction only achieves computational soundness, requires strong assumptions of quantum hardness of learning with errors (QLWE assumption) and the existence of quantum fully homomorphic encryption (QFHE), and relies on non-black-box simulation. In this paper, we resolve these issues at the cost of weakening the notion of zero-knowledge to what is called $\epsilon$-zero-knowledge. Concretely, we construct the following protocols: - We construct a constant round interactive proof for NP that satisfies statistical soundness and black-box $\epsilon$-zero-knowledge against quantum attacks assuming the existence of collapsing hash functions, which is a quantum counterpart of collision-resistant hash functions. Interestingly, this construction is just an adapted version of the classical protocol by Goldreich and Kahan (JoC '96) though the proof of $\epsilon$-zero-knowledge property against quantum adversaries requires novel ideas. - We construct a constant round interactive argument for NP that satisfies computational soundness and black-box $\epsilon$-zero-knowledge against quantum attacks only assuming the existence of post-quantum one-way functions. At the heart of our results is a new quantum rewinding technique that enables a simulator to extract a committed message of a malicious verifier while simulating verifier's internal state in an appropriate sense.

==> Simplified_ZK.tex <==
\section{Simplified Definition of Quantum $\epsilon$-Zero-Knowledge}
Here, we introduce a simplified weaker notion of quantum $\epsilon$-zero-knowledge which we call  \emph{quantum no-entanglement $\epsilon$-zero-knowledge}.
Roughly speaking, this ensures indistinguishability of real and simulated worlds only against distinguisher that is not given any state that is entangled to auxiliary input of the verifier and simulator.
Then we prove that quantum no-entanglement $\epsilon$-zero-knowledge implies quantum  $\epsilon$-zero-knowledge assuming a very mild condition on a simulator.
This enables us to focus on proving quantum no-entanglement $\epsilon$-zero-knowledge in the latter sections.

Our formal definitions of quantum no-entanglement $\epsilon$ zero-knowledge are given below:
\begin{definition}[Post-Quantum No-Entanglement  $\epsilon$-Zero-Knowledge Proof and Argument]
A post-quantum no-entanglement  $\epsilon$-zero-knowledge proof (resp. argument) for an NP language $\lang$ is a classical interactive proof (resp. argument) for $\lang$ that satisfies the following property (in addition to perfect completeness and statistical (resp. computational) soundness):
\paragraph{Quantum No-Entanglement $\epsilon$-Zero-Knowledge.}
For any noticeable function $\epsilon$, 
there exists a QPT simulator $\siml$ such that for any non-uniform QPT malicious verifier $\ver^*=\{\ver^*_\secpar,\rho_\secpar\}_{\secpar\in \mathbb{N}}$, we have
\[
\{\OUT_{\ver^*_\secpar}\execution{\pro(w)}{\ver^*_\secpar(\rho_\secpar)}(x)\}_{\secpar,x,w}
\compind_{\epsilon}
\{\siml(x,\ver^*_\secpar,\rho_\secpar)\}_{\secpar,x,w}
\]
where $\secpar \in \mathbb{N}$, $x\in \lang\cap \bit^\secpar$, $w\in \rel_\lang(\secpar)$.
\end{definition}

\begin{definition}[Quantum No-Entanglement  $\epsilon$-Zero-Knowledge Proof and Argument]\label{def:post_quantum_no_entanglement_ZK}
A quantum $\epsilon$-zero-knowledge proof (resp. argument) for a QMA language $\lang$ is a classical interactive proof (resp. argument) for $\lang$ that satisfies the following property (in addition to statistical completeness and statistical (resp. computational) soundness):
\paragraph{Quantum No-Entanglement  $\epsilon$-Zero-Knowledge.}
For any noticeable function $\epsilon$, 
there exists a QPT simulator $\siml$ such that for any non-uniform QPT malicious verifier $\ver^*=\{\ver^*_\secpar,\rho_\secpar\}_{\secpar\in \mathbb{N}}$, we have
\[
\{\OUT_{\ver^*_\secpar}\execution{\pro(w^{\otimes k(\secpar)})}{\ver^*_\secpar(\rho_\secpar)}(x)\}_{\secpar,x,w}
\compind_{\epsilon}
\{\siml(x,\ver^*_\secpar,\rho_\secpar)\}_{\secpar,x,w}
\]
where $\secpar \in \mathbb{N}$, $x\in \lang\cap \bit^\secpar$, $w\in \rel_\lang(\secpar)$.
\end{definition}
\begin{remark}
Bitansky and Shmueli \cite{STOC:BitShm20} used the ``non-entanglement" version as a default notion of quantum zero-knowledge.
However, we believe that this is slightly weaker than the orifinal definition by Watrous \cite{SIAM:Watrous09} in general.
%Fortunately, the quantum non-entanglement $\epsilon$-zero-knowledge implies the standard quantum $\epsilon$-zero-knowledge under a very mild condition about a simulator.
\end{remark}

In the following, we give a very mild sufficient condition so that quantum no-entanglement $\epsilon$-zero-knowledge implies the standard quantum  $\epsilon$-zero-knowledge.
\begin{lemma}\label{lem:no_entanglement_to_general_ZK}
Suppose that a classical/quantum interactive proof/argument satisfies
quantum no-entanglement $\epsilon$-zero-knowledge  w.r.t. a simulator $\siml$ that satisfies the following consdition:
\begin{itemize}
    \item If a circuit $\ver^*_\secpar(\rho_\secpar)$ trivially acts on some registers of $\rho_\secpar$, then $\siml(x,\ver^*_\secpar,\rho_\secpar)$ also trivially acts on these registers for any $x\in \bit^{\secpar}$.
\end{itemize}
Then the protocol also satisfies quantum  $\epsilon$-zero-knowledge.
\end{lemma}
\begin{proof}
We prove the lemma for classical protocols. The case of quantum protocols can be proven similarly.

Suppose that we have sequences $\{\ver^*_\secpar\}_{\secpar\in \mathbb{N}}$ and $\{\rho_\secpar\}_{\secpar\in \mathbb{N}}$ as in the definition of quantum $\epsilon$-zero-knowledge in Definition \ref{def:post_quantum_ZK}.
For each $\secpar$, we consider a modified circuit $\widetilde{\ver}^*_\secpar$ that works similarly to $\ver^*_\secpar$ except that it also takes a state on the register $\regR$ as part of its input, and also outputs that state as part of its output (without applying any operation on the register $\regR$).
Then clearly we have 
\[
(\Psi_{\real,\secpar,x,w}^{\ver^*}\otimes I_{\regR})(\rho_\secpar)
=
\OUT_{\widetilde{\ver}^*_\secpar}\execution{\pro(w^{\otimes k(\secpar)})}{\widetilde{\ver}^*_\secpar(\rho_\secpar)}(x)
\]
By quantum no-entanglement $\epsilon$-zero-knowledge, we have
\[
\{\OUT_{\widetilde{\ver}^*_\secpar}\execution{\pro(w^{\otimes k(\secpar)})}{\widetilde{\ver}^*_\secpar(\rho_\secpar)}(x)\}_{\secpar,x,w}\compind_\epsilon \{\siml(x,\ver^*_\secpar,\rho_\secpar)\}_{\secpar,x,w}
\]
where $\secpar \in \mathbb{N}$, $x\in \lang\cap \bit^\secpar$, $w\in \rel_\lang(\secpar)$.
Since $\ver^*$ trivially acts on the register $\regR$, $\siml(x,\ver^*_\secpar,\cdot)$ also trivially acts on $\regR$.
Therefore, we can define $\siml'$ that works similarly to $\siml$ except that it does not take a state in $\regR$ and does not output it. Then we have 
\[
\siml(x,\ver^*_\secpar,\rho_\secpar)=(\siml'(x,\ver^*_\secpar,\cdot)\otimes I_\regR)(\rho_\secpar).
\]
By combining the above, we can conclude that the protocol satisfies the quantum $\epsilon$-zero-knowledge property 
w.r.t. the simulator $\siml'$.
\end{proof}

==> WIPoK_from_OWF.tex <==
\section{Witness Indistinguishable Proof of Knowledge from OWF}\label{app:WIPoK_from_OWF}
In this section, we construct a constant round witness indistinguishable proof of knowledge based on any OWF. 
The construction is obtained by a slight tweak to the construction by Unruh \cite{EC:Unruh12} based on one-to-one OWF.
